Quantifying Membership Inference Risks in Genomic Data Sharing: The Role of Attacker's Auxiliary Information

Genomic data sharing is essential for biomedical research but introduces significant privacy risks, including membership inference attacks, in which an adversary determines whether a specific individual's data was used in a study. Existing privacy protections are typically applied after a release format has already been chosen, leaving researchers without a principled method to assess dataset-specific risk beforehand. We propose a server-assisted, principal component analysis-based pre-release auditing framework that maps genomic data into a shared low-dimensional space, applies epsilon-local differential privacy via the Laplace mechanism with a formally derived sensitivity for principal component analysis scores, and estimates membership inference attack power at a controlled 5% false-positive rate using a distance-threshold attack. A membership-neutrality diagnostic based on Unbiased Reconstruction Robustness is reported alongside attack power, precision, and recall. Experiments using the openSNP and 1000 Genomes Project datasets across multiple dimensionalities and privacy budgets show that separation between the researcher's dataset and public auxiliary data in principal component analysis space is a dominant determinant of attack success, exceeding the effect of perturbation level alone. Comparison against a genome-wide association study-style likelihood ratio test baseline further contextualizes the measured risk. This framework enables researchers, data repositories, and institutional review bodies to quantify dataset-specific membership inference risk before genomic data publication, supporting more informed and privacy-aware biomedical data-sharing decisions.

==> sections/Privacy_Analysis.tex <==
\section{Privacy Analysis}\label{sec:privacy}
In the proposed framework, although the researcher shares PCA-transformed data with Laplace noise, the server still represents a potential privacy risk, as discussed in Section~\ref{sec:system}. This section provides formal analysis of the privacy guarantees and residual risks in the framework.

\subsection{Formal LDP Guarantee}

The $\epsilon$-LDP guarantee of the framework rests on Proposition~\ref{prop:sensitivity}. In all experiments reported in this work, $\lambda$ is computed analytically from $\lambda = 2\sqrt{d}/\epsilon$, ensuring that all reported $\epsilon$ values correspond to rigorous formal guarantees. No empirical noise tuning is used.

\subsection{Server Leakage Bound}

The server receives both the DP-noised scores $\tilde{\mathbf{Y}}$ and the PCA model $(\mathbf{V}, \boldsymbol{\mu})$, which encodes population-level structure derived from $D_R$. The following proposition formally bounds the privacy risk introduced by sharing the PCA model. 

\begin{proposition}[\textbf{Server Leakage Bound}]
\label{prop:leakage}
A server attempting to recover individual genotype $\mathbf{x}_i$ from
DP-noised embedding $\tilde{\mathbf{y}}_i$ faces the inversion problem
$\hat{\mathbf{x}}_i = \tilde{\mathbf{y}}_i \cdot \mathbf{V}^{\dagger} +
\boldsymbol{\mu}$, where $\mathbf{V}^{\dagger}$ is the pseudoinverse of
$\mathbf{V}$. This system is severely underdetermined: with $d \leq 10$ and $p \geq 28{,}000$, the solution space has dimension $p - d \geq 27{,}990$.
DP noise bounds the expected reconstruction error as follows: 
\[
\mathbb{E}\bigl[\|\hat{\mathbf{x}}_i - \mathbf{x}_i\|_2\bigr]
\;\geq\; \lambda\sqrt{d} \;=\; \frac{2d}{\epsilon}.
\]
For $\epsilon = 1$ and $d = 2$, the expected reconstruction error exceeds $4$ units per individual, which is larger than the typical per-individual SNP variation range of $[0, 2]$ under normalized encoding.
\end{proposition}

The full proof is provided in Appendix~A. Note that this bound does not
constitute a cryptographic guarantee; the integration of secure multi-party computation protocols to eliminate the server trust assumption entirely is identified as a direction for future work.

\subsection{Privacy Composition Under Iterative Tuning}
\label{sec:composition}

The iterative nature of the proposed framework raises a DP composition concern: if a researcher submits $k$ risk queries with individual privacy budgets $\epsilon_1, \ldots, \epsilon_k$, the total privacy loss is bounded by $\epsilon_{\text{total}} = \sum_i \epsilon_i$ under basic composition~\cite{Dwork2014TheAlgorithmic}. Under advanced composition, this bound tightens to $\epsilon_{\text{total}} \approx \epsilon\sqrt{2k\log(1/\delta)} + k\epsilon(e^{\epsilon}-1)$ for $k$ queries at uniform $\epsilon$.

To manage this in practice, a \textit{privacy budget ledger} is recommended:
the researcher is assigned a total budget $\epsilon_{\text{budget}}$ prior to beginning the audit, and each server query consumes $\epsilon_i$ from this budget. The server enforces this limit and declines queries once the budget is exhausted. For $ \epsilon_{\text{budget}} = 10$ and $\epsilon_i = 1$
per query, up to $k = 10$ tuning rounds are supported before requiring a
held-out partition of $D_R$ with a fresh budget.

\subsection{Unbiased Reconstruction Robustness (U-ReRo)}
\label{sec:urero}

Traditional metrics for evaluating MIA robustness in differential privacy often overlook biases in reconstruction accuracy for members versus non-members. U-ReRo~\cite{Guerra2024Analysis} is a membership-neutral metric that evaluates the impact of DP mechanisms equally for both groups. U-ReRo measures the difference in reconstruction probabilities under a defined error threshold $\eta$, ensuring this difference remains below a tolerance $\gamma$.

\textbf{Instantiation in the proposed framework.}
Reconstruction of individual $i$ is defined as successful if the $\ell_2$ distance between the reconstructed score $\hat{\mathbf{x}}_i = \tilde{\mathbf{y}}_i \cdot \mathbf{V}^{\dagger} + \boldsymbol{\mu}$ and the true genotype $\mathbf{x}_i$ is below threshold $\eta = 0.5$. The following quantities are computed:
\begin{align*}
P_{\text{member}}    &= \bigl|\bigl\{i \in D_R :
                       \|\hat{\mathbf{x}}_i - \mathbf{x}_i\|_2 \leq \eta\bigr\}\bigr|
                       \;/\; |D_R|, \\
P_{\text{nonmember}} &= \bigl|\bigl\{j \notin D_R :
                       \|\hat{\mathbf{x}}_j - \mathbf{x}_j\|_2 \leq \eta\bigr\}\bigr|
                       \;/\; |D_\text{ref}|, \\
\text{U-ReRo}        &= |P_{\text{member}} - P_{\text{nonmember}}|.
\end{align*}

When $\text{U-ReRo} \leq \gamma = 0.5$, the mechanism is considered
membership-neutral. In the evaluation reported in this work, U-ReRo
consistently remained $\ll 0.1$, substantially below this threshold.

\subsection{Likelihood Ratio Test (LRT) Baseline}
\label{sec:lrt}

The privacy risk associated with sharing statistical metadata is also assessed by comparing against the standard practice of sharing GWAS statistics, as accepted by many institutions (e.g., NIH). Following the methodology of~\cite{Halimi2022Privacy,Sankararaman2009Genomic}, LRT values are computed using the minor allele frequencies (MAFs) of SNPs under null and alternate hypotheses. The null hypothesis assumes that a target individual $t$ is not part of the dataset, while the alternate hypothesis assumes membership. The overall LRT is:
\[
\text{LRT} = \sum_{s=1}^{\ell}
\left[z_{t,s} \log\frac{a_s}{\text{pop}_s}
+ (1 - z_{t,s})\log\frac{1-a_s}{1-\text{pop}_s}\right],
\]
where $z_{t,s}$ is the value of SNP $s$ for individual $t$, $a_s$ is the MAF of SNP $s$ in the dataset, $\text{pop}_s$ is the MAF of the same SNP in a reference population, and $\ell$ is the total number of released SNPs.

==> sections/Related_works.tex <==
\section{Related Work}\label{sec:Related_works}
The sharing of genomic data has accelerated biomedical research but has also introduced substantial privacy challenges, especially from MIAs, which attempt to infer whether an individual appears in a shared dataset. Prior work has proposed defenses that balance privacy and utility from multiple angles.

\textbf{Statistical Approaches to Privacy Risks:}
In \cite{Homer2008Resolving}, a statistical test showed that individuals can be detected in aggregate genomic datasets by comparing to external high-density genotype data, including inferring case/control membership in GWAS. This result helped motivate moving some GWAS outputs from open to controlled access, underscoring the need for privacy safeguards in genomic data sharing.

\textbf{Differential Privacy in Genomic Data:}
Differential privacy (DP) is a widely used framework for protecting sensitive data. \cite{chen2021Differential} studied DP defenses against MIAs for genomic ML models, finding that stronger privacy (smaller $\epsilon$) reduces accuracy in a roughly log-like manner and that sparsity/regularization can further reduce MIA vulnerability in high-dimensional settings.
In \cite{Sarathy2011Evaluating}, the authors analyzed Laplace noise for numeric datasets, highlighting utility--privacy trade-offs: in large datasets, Laplace noise may be insufficient for protection, while in small datasets the required noise can severely harm utility; they also note difficulties for skewed or unbounded data.
Building on DP for genomics, \cite{Yilmaz2022Genomic} proposed dependent local DP methods that exploit genomic correlations to improve utility while preserving privacy.

\textbf{Game-Theoretic and Statistical Modeling Approaches:}
\cite{zhang2024bayesnash} modeled publisher--adversary interactions as a Bayesian game, characterizing strategic noise addition that mitigates risk while maintaining utility.
In \cite{Halimi2022Privacy}, likelihood ratio tests (LRT) were used to quantify membership risk from shared minor allele frequencies (MAFs), providing a practical benchmark for evaluating privacy mechanisms.

\textbf{Vulnerabilities in Different Genomic Data Types:}
Humbert et~al. \cite{humbert2017Quantifying} showed that sharing familial SNP data can amplify privacy loss through kinship correlations and auxiliary sources.
Bu et~al. \cite{Bu2021Haplotype} demonstrated stronger membership inference using haplotypes, achieving high power without requiring the target's genome and enabling reconstruction of rare haplotypes from summary information.

\textbf{Metrics and Evaluation of Privacy Mechanisms:}
Guerra-Balboa et~al. \cite{Guerra2024Analysis} introduced U-ReRo to reduce bias in DP evaluations and assess whether protections are membership-neutral for both members and non-members. Hu et~al.~\cite{Hu2022Membership} surveyed MIAs broadly, emphasizing that defenses should be tailored to the data type and threat model.

Together, these studies motivate privacy mechanisms that account for realistic auxiliary information and dataset structure. The present work builds on this foundation by providing a pre-release auditing tool rather than a post-hoc defense, incorporating U-ReRo, and using PCA-based spatial analysis to evaluate how dataset proximity shapes privacy risk under practical privacy
budgets.

%The advent of machine learning (ML) models in various domains, while offering significant advancements in data processing and analytics, also presents notable privacy concerns. Among these, Membership Inference Attacks (MIAs) have emerged as a critical threat. MIAs aim to ascertain the presence of specific data records within the training dataset of an ML model. This poses substantial privacy risks, particularly in scenarios where the data pertains to sensitive information, such as individual health records or personal preferences. In their survey, Hongsheng Hu et al \cite{}. delve into the nuances of MIAs against machine learning models, offering a thorough classification based on the model's vulnerability, the attacker's knowledge level, and the methodologies employed in executing these attacks. The survey covers a broad spectrum of ML models, including both classification and generative models, and it delineates attack strategies in scenarios ranging from black-box to white-box access.

%The relevance of MIAs extends across various applications, from natural language processing to computer vision, underscoring the universal need for robust privacy-preserving mechanisms in ML. The survey highlights the susceptibility of both centralized and federated learning systems to MIAs, thereby amplifying the call for effective defense strategies. Although several defensive techniques have been proposed, the authors note the absence of a panacea that unequivocally prevents MIAs, marking an ongoing challenge in the field. Furthermore, their survey underscores potential future research directions, advocating for the development of more resilient defense mechanisms and the exploration of privacy implications within emerging ML paradigms. To aid in the advancement of research on MIAs, the authors have established an online resource repository, fostering a collaborative approach to addressing these critical privacy concerns.
